IRISformer: Dense Vision Transformers for Single-Image Inverse Rendering in Indoor Scenes

Indoor scenes exhibit significant appearance variations due to myriad interactions between arbitrarily diverse object shapes, spatially-changing materials, and complex lighting. Shadows, highlights, and inter-reflections caused by visible and invisible light sources require reasoning about long-range interactions for inverse rendering, which seeks to recover the components of image formation, namely, shape, material, and lighting. In this work, our intuition is that the long-range attention learned by transformer architectures is ideally suited to solve longstanding challenges in single-image inverse rendering. We demonstrate with a specific instantiation of a dense vision transformer, IRISformer, that excels at both single-task and multi-task reasoning required for inverse rendering. Specifically, we propose a transformer architecture to simultaneously estimate depths, normals, spatially-varying albedo, roughness and lighting from a single image of an indoor scene. Our extensive evaluations on benchmark datasets demonstrate state-of-the-art results on each of the above tasks, enabling applications like object insertion and material editing in a single unconstrained real image, with greater photorealism than prior works. Code and data are publicly released at https://github.com/ViLab-UCSD/IRISformer.

==> Sections/Method_bak.tex <==
\section{Method}
\label{sec:method}

\noindent\textbf{Notation.}
Vectors are represented with a lower-case bold font (\eg $\mathbf{x}$). Matrices are in upper-case bold (\eg $\mathbf{X}$) while scalars are in regular font (\eg $x$ or $X$). 
% For indexing into a matrix, we use subscripts (\eg $\mathbf{M}_\mathbf{x}$).
Variables with hat, \eg $\mathbf{\hat X}$, are the estimation of the corresponding entity $\mathbf{X}$. For denoting the $l^{th}$ sample in a set (\eg images, shapes), we use subscripts (\eg $\mathbf{X}_{l}$). Uppercase calligraphic symbols (\eg$\mathcal{X}$) denote functions. 

\subsection{Scene Representation and Loss Functions}
\noindent\textbf{Geometry and spatially-varying material.} 
In our model, we account for only the scene elements within the camera frustum. For an $h \times w$ image, we represent per-pixel geometry with a depth map $\mathbf{D} \in \mathbb{R}^{h\times w}$ and normals $\mathbf{N} \in \mathbb{R}^{h\times w \times 3}$. We represent material as a microfacet spatially-varying BRDF model (SVBRDF)~\cite{karis2013svbrdf}, with albedo $\mathbf{A}$ and roughness $\mathbf{R}$ maps of sizes $h \times w \times 3$ and $h \times w$ respectively. Specifically, given a single RGB input image $\mathbf{I}$, we seek to learn a function \textbf{BRDFGeoNet} denoted as $\mathcal{B}$ to jointly estimate the above properties: $\{\mathbf{\hat D}, \mathbf{\hat N}, \mathbf{\hat A}, \mathbf{\hat R}\} = \mathcal{B}(\mathbf{I})$.
% \begin{equation}
%     \{\mathbf{\hat D}, \mathbf{\hat N}, \mathbf{\hat A}, \mathbf{\hat R}\} = \mathcal{B}(\mathbf{I}).
% \end{equation}
Given ground truths, we use scale-invariant L2 loss~\cite{li2020inverse, ranftl2019midas} for albedo and depth ($\log$ space) and an L2 loss for roughness and normals.

\vspace{0.2cm}
\noindent\textbf{Spatially-varying lighting.}
For lighting, we follow Li~\etal~\cite{li2020inverse} to adopt per-pixel image-space environment maps to $\mathcal{G}$ to represent the incident irradiance, parameterized by $K=12$ Spherical Gaussian (SG) lobes $\{\xi_k, \lambda_k, \textbf{f}_k\}_{k=1}^{K}$. Here $\xi_k \in \mathbb{S}^2$ is the center orientation on the unit sphere, $\textbf{f}_k \in \mathbb{R}^3$ is the intensity and $\lambda_k \in \mathbb{R}$ is the bandwidth. Given each set of lighting parameters and an orientation outward from one spatial location $\eta$ in 3D, we have
\begin{equation}
    \mathcal{G}(\eta) = \sum_{k=1}^{K} \textbf{f}_k e^{\lambda (1 - \eta \xi)}:\mathbb{S}^2 \rightarrow \mathbb{R}^3.
\end{equation}
We adopt an environment map resolution of $16 \times 32$ for each pixel location. For a collection of all $h\times w$ pixel locations and all $16\times 32$ outgoing directions from each surface point in 3D, we arrive at a lighting map $\mathbf{L} \in \mathbb{R}^{h \times w \times 16 \times 32 \times 3}$. Then, using either a single image as the sole input or combining it with predictions of geometry and material, a \textbf{LightNet} denoted as $\mathcal{L}$ can be learned: $\mathbf{\hat L} = \mathcal{L}(\mathbf{I})$ or $\mathbf{\hat L} = \mathcal{L}(\mathbf{I}, \mathbf{\hat D}, \mathbf{\hat N}, \mathbf{\hat A}, \mathbf{\hat R})$.
% \begin{equation}
%     \mathbf{\hat L} = \mathcal{L}(\mathbf{I}), \; {\textrm{ or }}
%     \mathbf{\hat L} = \mathcal{L}(\mathbf{I}, \mathbf{\hat D}, \mathbf{\hat N}, \mathbf{\hat A}, \mathbf{\hat R}).
% \end{equation}
%
Given estimates of geometry, material and lighting, a per-pixel physically-based differentiable renderer \textbf{RenderNet}~\cite{li2020inverse} denoted as $\mathcal{R}$ can re-render the input image: $\mathbf{\hat I} = \mathcal{R}(\mathbf{\hat D}, \mathbf{\hat N}, \mathbf{\hat A}, \mathbf{\hat R}, \mathbf{\hat L})$.
% \begin{equation}
%     \mathbf{\hat I} = \mathcal{R}(\mathbf{\hat D}, \mathbf{\hat N}, \mathbf{\hat A}, \mathbf{\hat R}, \mathbf{\hat L}).
% \end{equation}
%

To supervise training of lighting, assuming dense ground truth can be acquired from synthetic datasets, we impose a scale-invariant L2 reconstruction loss on the lighting map $\mathbf{\hat L}$ (in $\log$ space) and a scale-invariant L2 re-rendering loss on the re-rendered image $\mathbf{\hat I}$. The final loss $L_{all}$ is a weighted combination of losses on all estimations: 

\begin{equation}
    L_{all} = \lambda_{\textbf{A}} L_{\textbf{A}} + \lambda_{\textbf{R}} L_{\textbf{R}} + \lambda_{\textbf{D}} L_{\textbf{D}} + \lambda_{\textbf{N}} L_{\textbf{N}} + \lambda_{\textbf{L}} L_{\textbf{L}} + \lambda_{\textbf{I}} L_{\textbf{I}}.
    \label{equ:loss}
\end{equation}

% \noindent\textbf{Material representation.}
\begin{figure*}
\centering
\includegraphics[width=0.95\textwidth]{Figures/OR_results.pdf}
\vspace{-0.2cm}
\caption{BRDF, geometry and lighting estimation on OpenRooms. Small insets (best viewed when enlarged in PDF version) are estimations processed with bilateral solvers (BS). More results can be found in the supplementary material.}
\vspace{-0.4cm}
\label{fig:or_results}
\end{figure*}


% \noindent\textbf{Vision transformer.}
\subsection{Dense Vision Transformer}
Dense Vision Transformer (DPT)~\cite{ranftl2021dpt} is a generic architecture for dense prediction utilizing vision transformers~\cite{dosovitskiy2020vit} in place of CNNs as a backbone. An image $\mathbf{I}$ is first divided into an $h/p \times w/p$ grid of non-overlapping patches of size $p\times p$, and subsequently DPT tokenizes each patch into a vector of dimension $D$ with a shadow CNN (DPT-large or DPT-base) or ResNet (DPT-hybrid). The result is a set of tokens $\textbf{t}^0 = \{\textbf{t}^0_1, \hdots, \textbf{t}^0_{N_p}\}$ where $N_p = hw/p^2$, $\textbf{t}^0_n \in \mathbb{R}^D, n=[1, \dots N_p]$. A cascade of $M$ transformer layers then transforms the set of vectors with self-attention~\cite{vaswani2017attention} into $\textbf{t}^M$, and a re-assembling operation followed by a convolutional decoder transforms the tokens back to 2D space, resulting in a 2D dense feature map. A customized convolutional head is attached to yield the final prediction from the feature map, based on the specific prediction task. In our case, we use an input resolution of 256$\times$320 and patch size $p=16$. 

\subsection{Single-task Network Design}
Due to the modular design of DPT and the variation of size and capacity among different DPT models, we consider a few design choices for using DPT modules to build our \textbf{BRDFGeoNet} and \textbf{LightNet} in both single-task and multi-task settings. In single-task setting, we seek to maximize the performance of each task by using an independent DPT for each of depth, normal, albedo, roughness. This effectively results in \textbf{BRDFGeoNet} of 4 DPTs: $\mathbf{D} = \mathcal{B}_D(\mathbf{I})$, $\mathbf{N} = \mathcal{B}_N(\mathbf{I})$, $\mathbf{A} = \mathcal{B}_A(\mathbf{I})$, $\mathbf{R} = \mathcal{B}_R(\mathbf{I})$. For each DPT, we follow the design of DPT-hybrid~\cite{ranftl2021dpt} by using $M=6$ transformer layers for encoding and $M=6$ for decoding. A ResNet-50~\cite{he2016deep} acts as the patch embedding backbone. Readout token~\cite{ranftl2021dpt} is set to \textit{ignore} and batch normalization (BN) is enabled in output heads.
% and we choose not to use the read-out token, since we find it to have a minimal effect in the case of dense prediction. 
Details on the tensor sizes and head design are in the supplementary material.

\subsection{Multi-task Network Design}

The full design of our pipeline can be found in Fig.~\ref{fig:pipeline}. 
The single-network design requires 4 DPTs for material and geometry and one for lighting. As a result, the collective memory footprint is too large to fit the entire model into a regular GPU for training. An alternative option is to allow DPTs to have a unified feature space so that memory usage can be reduced. Also in some cases, a jointly learned feature can benefit related tasks. Inspired by UniT~\cite{hu2021unit} where input-domain-specific encoders and shared decoders are designed for a multi-modal input setting, we use a unified encoder and decoder for all tasks in \textbf{BRDFGeoNet} besides independent task-specific convolutional heads. We share decoders due to memory considerations, while noting that further gains from independent decoders might be possible.
%\rui{... we are sharing decoders; but no experiment was done VS indept decoders because of memory issue...}.

For \textbf{LightNet}, three independent heads are required for estimating axis center, intensity, and bandwidth of $K$ Spherical Gaussians for each pixel. However we found that sharing decoders for the three tasks is not optimal as the output spaces of these tasks are very disparate, thus forcing a unified decoder feature space destabilizes training. As a result, we use a shared encoder but independent decoders and output heads for \textbf{LightNet}. We use 4 transformer layers in both encoders and decoders in the multi-task setting so that the entire model can fit into one GPU for joint training.

\subsection{Additional Components}
\noindent{\textbf{Refinement using bilateral solver.}} 
We may optionally refine the geometry and material outputs with a bilateral solver (BS). Additional refinement leads to smoother outputs, which is preferable for some metrics like WHDR~\cite{bell2014iiw} for albedo. In comparison to previous works, we observe that our transformer-based outputs are already quite accurate without the bilateral solver on all the tasks.

%Similar to Li \etal~\cite{li2020inverse}, we also attempted including bilateral solvers for adaptively processing estimations for albedo, roughness and depth before they are fed into \textbf{LightNet}. We will include results with bilateral solver in the evaluation but we did not use bilateral solver to process results from \textbf{BRDFGeoNet} before they are fed into \textbf{LightNet} because bilateral solver brings unwanted artifacts to the our estimation, and little impact on the final performance.

\vspace{0.2cm}
\noindent{\textbf{Cascade design.}} In prior works~\cite{li2020inverse}, a cascade design is used to refine the predictions based on the rendering error. However, it leads to a two-fold increase in memory with small improvements, while we already achieve significantly improved results on all benchmarks with a single-stage network. As a result, we choose not to use cascaded refinement.


